Graph Auto-Encoder Via Neighborhood Wasserstein Reconstruction

Graph neural networks (GNNs) have drawn significant research attention recently, mostly under the setting of semi-supervised learning. When task-agnostic representations are preferred or supervision is simply unavailable, the auto-encoder framework comes in handy with a natural graph reconstruction objective for unsupervised GNN training. However, existing graph auto-encoders are designed to reconstruct the direct links, so GNNs trained in this way are only optimized towards proximity-oriented graph mining tasks, and will fall short when the topological structures matter. In this work, we revisit the graph encoding process of GNNs which essentially learns to encode the neighborhood information of each node into an embedding vector, and propose a novel graph decoder to reconstruct the entire neighborhood information regarding both proximity and structure via Neighborhood Wasserstein Reconstruction (NWR). Specifically, from the GNN embedding of each node, NWR jointly predicts its node degree and neighbor feature distribution, where the distribution prediction adopts an optimal-transport loss based on the Wasserstein distance. Extensive experiments on both synthetic and real-world network datasets show that the unsupervised node representations learned with NWR have much more advantageous in structure-oriented graph mining tasks, while also achieving competitive performance in proximity-oriented ones.

==> old02relatedworks.tex <==
\section{Related Work}


\textbf{Graph neural networks.}
GNNs have drawn significant research attention recently \citep{wu2020comprehensive,nikolentzos2020random,nikolentzos2020random,zhu2020beyond,balcilar2021analyzing,chien2021adaptive}. 
We focus on a particular yet generic family in this work, that is, message passing GNNs \citep{gilmer2017neural}, which includes arguably the most popular ones such as GCN \citep{kipf2016semi}, GraphSage \citep{hamilton2017inductive}, SGC \citep{wu2019simplifying}, GIN \citep{xu2018powerful}, GAT \citep{velivckovic2017graph}, PPNP \citep{klicpera2018predict} and so on. 
Equipped with slightly different message passing and aggregation functions, they essentially aim to encode complex node features and link structures in the local neighborhood of each node into a low-dimensional embedding vector, i.e., a $k$-layer GNN encodes the $k$-hop neighborhood \citep{huang2020graph}. 
The various message passing GNNs have been shown to enjoy provably strong representation power \citep{xu2018powerful,keriven2019universal,azizian2021expressive} and empirically superior task performance \citep{hamilton2017inductive,velivckovic2017graph,ying2018hierarchical}.
However, these GNNs often need to be trained with task-specific supervision. \pan{This para can be moved entirely to appendix}

%unsupervised GraphSAGE~\citep{hamilton2017inductive}, GAE~\citep{kipf2016variational}, their generative variants such as VGAE~\citep{kipf2016variational}, Graphite~\citep{grover2019graphite}, and many others~\citep{pan2018adversarially,shi2020effective}

\textbf{Unsupervised graph representation learning.}
Network embedding methods such as DeepWalk \citep{perozzi2014deepwalk}, LINE \citep{qiu2018network} and node2vec \citep{grover2016node2vec} are naturally unsupervised, but they are transductive (unable to be transferred or generalized to new data) and mostly proximity-driven. %\pan{Be careful when saying transductive. I prefer to say them limited to un-attributed graphs}
To train GNNs without task-specific supervision, auto-encoder based frameworks like unsupervised GraphSAGE~\citep{hamilton2017inductive}, GAE \citep{kipf2016variational}, VGAE \citep{kipf2016variational}, graphVAE \citep{simonovsky2018graphvae} and others \citep{wang2017mgae,pan2018adversarially,li2020dirichlet,grover2019graphite,shi2020effective} have been widely explored, but they are also strongly proximity-driven, and their link reconstruction decoders do not facilitate the preservation of complex and higher-order structure information in the neighborhoods. 
DGI~\citep{velivckovic2018deep}, InfoGraph \citep{sun2019infograph} and others~\citep{hu2019strategies,you2020graph,hassani2020contrastive} based on constrasive learning are by far the only unsupervised GNN training methods that consider graph structures beyond direct links. However, they adopt the rule of mutual information maximization, which essentially works to maximize certain correspondence between the learned representations and the original data. For example, DGI~\citep{velivckovic2018deep} and InfoGraph \citep{sun2019infograph} maximize the correspondence between a node representation and which graph the node belongs to, which still has no guarantee to reconstruct the structure information of node neighborhoods. Recent works also demonstrate that maximizing such correspondence indeed does not capture the full neighborhood information~\citep{tschannen2019mutual}, which is demonstrated again by our experiments. 


%their maximization of the mutual information between local node embedding and global graph embedding essentially enforces the GNN encoders to produce consistent embeddings for nodes in the same graph, instead of helping the GNN encoders to fully capture the local neighborhood information.

\textbf{Optimal-transport (OT) losses.} Many machine learning problems depend on characterization of the distance between two probability measures. The family $f$-divergence has the non-continuous issue when the two measures of interest have non-overlapped support~\citep{ali1966general}. Therefore, OT losses are often adopted and have shown great success in generative models~\citep{gulrajani2017improved} and domain adaptation~\citep{courty2016optimal}. OT-losses have been used to build variational auto-encoders for non-graph data~\citep{tolstikhin2018wasserstein,kolouri2018sliced,patrini2020sinkhorn}. But one should note the our work is not a graph-data-oriented generalization of these works: They use OT losses to characterize the distance between the variational distribution and the data empirical distribution while our model even does not have a variational distribution. Our model may be further improved by being reformulated as a variational autoencoder but we leave it as a future direction. 

Here, we give a frequently-used OT loss based on 2-Wasserstein distance that will be used later.
\begin{definition}
Let $\mathcal{P},\mathcal{Q}$ denote two probability distributions with finite second moment defined on $\mathcal{Z}\subseteq \mathbb{R}^m$. The $2$-Wasserstein distance between $\mathcal{P}$ and $\mathcal{Q}$ defined on $\mathcal{Z}, \mathcal{Z}'\subseteq \mathbb{R}^m$  is the solution to the optimal mass transportation problem with $\ell_2$ transport cost \citep{villani2008optimal}:
\begin{align} \label{eq:w-dis}
    \mathcal{W}_2(\mathcal{P},\mathcal{Q}) = \left( \inf_{\gamma \in \Gamma(\mathcal{P},\mathcal{P})} \int_{\mathcal{Z}\times \mathcal{Z}'} \|Z-Z'\|_2^2 d\gamma(Z, Z') \right)^{1/2}
\end{align}
where $\Gamma(\mathcal{P},\mathcal{Q})$ contains all joint distributions of $(Z, Z')$ with marginals $\mathcal{P}$ and $\mathcal{Q}$ respectively. %$\Gamma(\mathcal{P}^{(i)},\mathcal{P}^{(j)})$ is the set of all transportation plans $\gamma \in \Gamma(\mathcal{P}^{(i)},\mathcal{P}^{(j)})$ such that $\gamma()$
\end{definition}




%Our neighborhood reconstruction is related to the recent graph

%Our auto-encoder includes the reconstruction of neighbor-representation distributions, which needs to measure the distance between probability measures. Traditional $f$-divergence 

%\pan{para 2: related techniques: kl divergence, mutual information, wasserstein, hungarian, sinkhorn autoencoder (we are not variational)}\\

==> old03method.tex <==


\section{Methods}
\subsection{Motivations \& Other Related Works: Neighbor Information Reconstruction}  \label{sec:prelim}
%\pan{some parts may be removed due to the overlapping with intro. put GNN encoder in related work. fix gaps.}

In this work, we focus on the auto-encoder framework for unsupervised task-agnostic graph representation learning, which is preferred in abundant learning scenarios where labeled data are unavailable and/or generalizable and transferable representations are in need.

The original motivation of auto-encoders is to perform neural-network-based dimension reduction of the data that originally lies in a high-dimensional space~\citep{hinton2006reducing}. Specifically, an auto-encoder consists of two components, an encoder and a decoder. The encoder works to compress each data point into a low-dimensional vector representation, while the decoder works to reconstruct the original information from this vector. By minimizing the reconstruction error, the encoder automatically converges to a good compressor that allows the low-dimensional representations to capture as much information as possible from the original data.  

Although the above high-level idea of auto-encoders is clear, when it is applied to graph structured data, the problem becomes challenging. This is because in graph-structured data, information of data points (nodes to be specific as most widely studied) is correlated due to the ambient graph structure. Without specific task need in a priori, the learned low-dimensional representation of a node should carry as much information as possible from not only its own features but also the features of the nodes it connects to (both directly and indirectly). 
%What information should be compressed into their low-dimensional representations is not clearly defined. %opinions on what information should be reconstructed seem to be divergent from such a motivation. 
%This leads to a

%This implies that when building auto-encoders for graph-structure data, we expect the node representations to be able to reconstruct all correlated node features. However, existing graph auto-encoders seem to be away from this motivation. Without exception, they adopt link reconstruction in the decoder as the main drive to optimize their GNN encoders.
%which as a result limits the information that the learned node representations actually capture. 

This implies that when building auto-encoders for graph-structure data, we expect the node representations to be able to reconstruct all correlated node features. However, existing graph auto-encoders seem to be away from this motivation, which as a result limits the information that the learned node representations actually capture.   
Previous prominent works such as unsupervised GraphSAGE~\citep{hamilton2017inductive}, GAE~\citep{kipf2016variational}, their generative variants such as VGAE~\citep{kipf2016variational}, Graphite~\citep{grover2019graphite}, and many others~\citep{pan2018adversarially,shi2020effective}, use graph convolutional networks (GNNs) to encode graph structured data into node representations. Without exception, they adopt link reconstruction in the decoder as the main drive to optimize their GNN encoders. The node representations obtained in this way essentially transform node features to best record the network linkage information but lose much of other important information, such as local structures, neighbors' features, etc. These auto-encoders give valid node representations when link prediction is the downstream task, but they will most likely fail in other tasks such as node classifications (especially structure-oriented ones as manifested in Figure \ref{fig:toy_example}).

%\pan{We probably want to introduce encoder here.}

To better understand this point, we carefully analyze the source of information encoded in each node representation via a GNN. Suppose a standard message passing GNN~\citep{gilmer2017neural} is adopted as the encoder, which is a general framework that includes GCN~\citep{kipf2016semi}, GraphSAGE~\citep{hamilton2017inductive}, GAT~\citep{velivckovic2017graph}, GIN~\citep{xu2018powerful} and so on. After $k$-hop message passing, the source of information encoded in the representation of a node $v$ essentially comes from the $k$-hop neighborhood of $v$ (Fig.~\ref{fig:info-source}). Therefore, a good representation of node $v$ should capture the information of features from all nodes in its $k$-hop neighborhood, which is agnostic to downstream tasks. Note that this may not be ideal as nodes out of $k$-hop neighborhood may also provide useful information, but this is what GNN-based graph auto-encoders can be expected to do due to the their architectures of GNN encoders. This observation motivates our study on a novel graph decoder that can better facilitate the goal of GNN-based graph auto-encoders, based on the following neighborhood reconstruction principle.

\begin{figure}[t]
\centering
    \includegraphics[trim={0.7cm 14.1cm 7.5cm 3.3cm},clip,width=0.9\textwidth]{figures/info-source.pdf}
    \vspace{-0.1cm}
    \caption{The information source/receptive field of the node representation $h_v^{(2)}$.}
    \label{fig:info-source}
\end{figure}
\begin{figure}[t]
\centering
    \includegraphics[trim={3.7cm 9.cm 2.1cm 3.3cm},clip,width=\textwidth]{figures/diagram.pdf}
    \vspace{-0.5cm}
    \caption{The diagram of our model using an example with 2 GNN layers as the encoder.}
    \label{fig:model}
\end{figure}

\subsection{Neighborhood Reconstruction Principle (NRP)}  \label{sec:principle}
%To simplify the exposition, we start from 1-hop neighborhood reconstruction and later generalize the notion to $k$-hop setting.
Let $G = (V, E, X)$ denote the input graph where $V$ is the node set, $E$ is the edge set and $X=\{x_v|v\in V\}$ includes the node features. Given a node $v\in V$, we define its $k$-hop neighborhood as the nodes which have shortest paths of length no greater than $k$ from $v$. Let $\mathcal{N}_v$ denote the 1-hop neighborhood of $v$, and $d_v$ denote the degree of node $v$. %$^{(k)}=\{u\in V| l(u,v)\leq k\}$, where $l(\cdot,\cdot)$ denotes the shortest path distance. %Denote the induced $k$-hop subgraph based on $\mathcal{N}_v^{(k)}$ as $G_v^{(k)}$.

We are to build an auto-encoder to learn a low-dimensional representation of each node. Specifically, the auto-encoder will have an encoder $\phi$ and a decoder $\psi$. $\phi$ could be any message-passing GNNs~\citep{gilmer2017neural}. The decoder further contains three parts $\psi=(\psi_s,\psi_p,\psi_d)$. The physical meaning of each part will be clear as we introduce them in the later subsections. %The specific forms of different parts of $\psi$ will be introduced in subsections later while temporarily we view them as general neural network models.

\textbf{First-hop neighborhood reconstruction.} To simplify the exposition, we start from $1$-hop neighborhood reconstruction. We initialize the node representation by $H^{(0)}$ based on $X$. % (Eq.\eqref{eq:ini} which will be explained later). 
For every node $v\in V$, after encoded by one GNN layer, its node representation $h_v^{(1)}$ collects information from $h_v^{(0)}$ and its neighbors' representations $H^{(0)}_{\mathcal{N}_v} = \{h_u^{(0)}|u\in \mathcal{N}_v\}$. Hence, we consider the following principle that reconstructs the information from both $h_v^{(0)}$ and $H^{(0)}_{\mathcal{N}_v}$. Therefore, we have
\begin{align}\label{eq:obj-1hop}
    \min_{\phi,\psi} \sum_{v\in V} \mathcal{M}((h_v^{(0)}, H^{(0)}_{\mathcal{N}_v}), \psi(h_v^{(1)})), \quad \text{s.t.}\; h_v^{(1)} = \phi(h_v^{(0)}, H^{(0)}_{\mathcal{N}_v}), \,\forall v\in V
\end{align}

where $\mathcal{M}(\cdot, \cdot)$ defines the reconstruction loss. $\mathcal{M}$ can be split into two parts that measure self-feature reconstruction and neighborhood reconstruction respectively.    
\begin{align} \label{eq:split}
    \mathcal{M}((h_v^{(0)},H^{(0)}_{\mathcal{N}_v}), \psi(h_v^{(1)})) = \mathcal{M}_s(h_v^{(0)}, \psi(h_v^{(1)}))+ \mathcal{M}_{n}(H^{(0)}_{\mathcal{N}_v}, \psi(h_v^{(1)})).
\end{align}
Note that $\mathcal{M}_s$ works just as the reconstruction loss of a standard feedforward neural network (FNN)-based auto-encoder, so we adopt
\begin{align} \label{eq:self-loss}
    \mathcal{M}_s(h_v^{(0)}, \psi(h_v^{(1)})) = \|h_v^{(0)} - \psi_s(h_v^{(1)})\|^2.
\end{align}
$\mathcal{M}_{n}$ is much harder to characterize, as it measures the loss to reconstruct a set of features $H^{(0)}_{\mathcal{N}_v}$. There are two fundamental challenges: First, as in real-world networks the distribution of node degrees is often long-tailed, the sets of node neighbors may have very different sizes. Second, to compare even two equal-sized sets, a matching problem has to be solved, as no fixed orders of elements in the sets can be assumed. The complexity to solve a matching problem is high if the size of the set is large. We solve the above challenges via two steps: First, we decouple the neighborhood information into a probability distribution and a sampling number. Specifically, for node $v$ % We term this neighborhood information decomposition (NID): \\
the neighborhood information is represented as an empirical realization of \text{i.i.d.} sampling $d_v$ elements from $\mathcal{P}_v^{(0)}$, where $\mathcal{P}_v^{(0)}\triangleq \frac{1}{d_v}\sum_{u\in \mathcal{N}_v} \delta_{h_u^{(0)}}$. Based on this view, we are able to decompose the reconstruction into the part for the node degree and that for the distribution respectively, where the various sizes of node neighborhoods are handled properly. Specifically, we adopt 
\begin{align} \label{eq:neighbor-loss}
    \mathcal{M}_{n}(H^{(0)}_{\mathcal{N}_v}, \psi(h_v^{(1)})) = (d_v - \psi_d(h_v^{(1)}))^2 + \mathcal{W}_2^2(\mathcal{P}_v^{(0)}, \psi_p^{(1)}(h_v^{(1)})),
\end{align}
where $\mathcal{W}_2(\cdot,\cdot)$ is the 2-Wasserstein distance as defined in Eq.\eqref{eq:w-dis}. % the distribution $\mathcal{P}_v^{(0)}$ reconstruction. %We will discuss it in Sec.~\ref{sec:w-dis}. 
Plug Eqs.\eqref{eq:self-loss}\eqref{eq:neighbor-loss} into Eq.\eqref{eq:split}, we obtain the objective for first-hop neighborhood reconstruction.

\textbf{Generalizing to $k$-hop neighborhood reconstruction.} Following the above derivation for the first-hop case, one can similarly generalize the loss for reconstructing $(h_v^{(i-1)},H^{(i-1)}_{\mathcal{N}_v})$ based on $h_v^{(i)}$ for all $1\leq i \leq k$. Then, if we sum such losses over all nodes $v\in V$ and all hops $1\leq i\leq k$, we may achieve the objective for $k$-hop neighborhood reconstruction. We may further simplify such an objective. Typically, only the final layer representation $H^{(k)}$ is used as the output dimension-reduced representations. %but they are not directly related to initial features $H^{(0)}$ in the construction loss. 
Too many intermediate hops make the model hard to train and slow to converge. Therefore, we adopt a more economic way by merging the multi-step reconstruction: 
%\includegraphics[trim={1.7cm 15.4cm 9.4cm 4.5cm},clip,width=0.8\textwidth]{simplification.pdf}\\
\begin{figure}[h]
    \centering
    \includegraphics[trim={1.7cm 15.4cm 9.4cm 4.5cm},clip,width=0.8\textwidth]{figures/simplification.pdf}
    \vspace{-0.3cm}
    %\caption{Causal anonymous walks (CAW): causality extraction and set-based anonymization.}
    %\vspace{-0.5cm}
    %\label{fig:s}
\end{figure}
%$h_v^{(k)}\rightarrow h_v^{(k-1)} \rightarrow \cdots \rightarrow h_v^{(i)}\rightarrow  (h_v^{(i-1)},H^{(i-1)}_{\mathcal{N}_v})$ into one step $h_v^{(k)}\rightarrow (h_v^{(i-1)},H^{(i-1)}_{\mathcal{N}_v})$ for $i\in [1, k-1]$. %Such simplification is reasonable because $h_v^{(k)}$ contains the information (possibly compressed) from $h_v^{(i)}$ and one may view  . 

That is, we expect $h_v^{(k)}$ to directly reconstruct $H^{(i)}_{\mathcal{N}_v}$ even if $i<k-1$. Specifically, for each node $v\in V$, we use the reconstruction loss
\begin{align} \label{eq:k-hop-loss}
    \mathcal{M}'&((h_v^{(0)},\{H^{(i)}_{\mathcal{N}_v}|0\leq i\leq k-1\}), \psi(h_v^{(k)})) =  \mathcal{M}_s(h_v^{(0)}, \psi(h_v^{(k)})) + \sum_{i=0}^{k-1} \mathcal{M}_{n}(H^{(i)}_{\mathcal{N}_v}, \psi(h_v^{(k)})) \nonumber \\
    &=\lambda_s \|h_v^{(0)}- \psi_s(h_v^{(k)})\|^2 + \lambda_d (d_v - \psi_d(h_v^{(k)}))^2 
    + \sum_{i=0}^{k-1}\mathcal{W}_2^2(\mathcal{P}_v^{(i)}, \psi_p^{(i)}(h_v^{(k)})),  
\end{align}
where $\psi_s$ is to decode the initial features, $\psi_d$ is to decode the degree and $\psi_p^{(i)}$, $0\leq i \leq k-1$ is to decode the $i$-layer neighbor representation distribution $\mathcal{P}_v^{(i)}(:\triangleq \frac{1}{d_v}\sum_{u\in \mathcal{N}_v} \delta_{h_u^{(i)}})$. $\lambda_s$ and $\lambda_d$ are non-negative hyperparameters. Hence, the entire objective for $k$-hop neighborhood reconstruction is 
\begin{align} \label{eq:k-hop-obj}
    \min_{\phi, \psi} \sum_{v\in V}\mathcal{M}'&((h_v^{(0)},\{H^{(i-1)}_{\mathcal{N}_v}|1\leq i\leq k\}), \psi(h_v^{(k)})) \quad \text{s.t.}\; H^{(i)} = \phi^{(i)}(H^{(i-1)}), 1\leq i\leq k,
\end{align}
where $\phi = \{\phi^{(i)}| 1\leq i\leq k\}$ include $k$ GNN layers and $\mathcal{M}'$ is defined in Eq.\eqref{eq:k-hop-loss}.

\begin{remark}
The loss in Eq.~\eqref{eq:k-hop-loss} does not directly push the $k$-layer representation $h_v^{(k)}$ to reconstruct the features of all nodes that are direct neighbors but lie in $k$-hop neighborhood of $v$. %, say $h_u^{(0)}$, if $u$ is not a direct neighbor but lies in $k$-hop neighborhood of $u$. 
However, by definition, there exists a shortest path of length no greater than $k$ from $v$ to every node in this $k$-hop neighborhood. As every two adjacent nodes along the path will introduce at least one term of reconstruction loss in the sum of Eq.~\eqref{eq:k-hop-loss}, i.e., the objective in Eq.~\eqref{eq:k-hop-obj}, this guarantees that the optimization in Eq.~\eqref{eq:k-hop-obj} pushes $h_v^{(k)}$ to reconstruct the entire $k$-hop neighborhood of $v$.
\end{remark}

\subsection{Decoding Distributions based on Wassertein Distance --- Decoders $\psi_p^{(i)}$, $0\leq i \leq k-1$} \label{sec:w-dis}
One important simplification adopted by our NRP is to represent the node neighborhood $H^{(i)}_{\mathcal{N}_v}$ as a sampling number (node degree $d_v$) plus a distribution of neighbors' representations $\mathcal{P}_v^{(i)}$ (Eqs.\eqref{eq:neighbor-loss}\eqref{eq:k-hop-loss}). We adopt Wasserstein distance to characterize the distribution reconstruction loss because $\mathcal{P}_v^{(i)}$ has atomic non-zero measure supports in a continuous space, where the family of $f$-divergence are not applied. Note that 2-Wassertein distance as we adopt is not crucial and other OT losses may be used as well.    

We set the decoded distribution $\psi_p^{(i)}(h_v^{(k)})$ as an FNN-based transformation of a Gaussian distribution parameterized by $h_v^{(k)}$. Here, the reparameterization trick needs to be used ~\citep{kingma2014autoencoding}, i.e.,
\begin{align*}
    \psi_p^{(i)}(h_v^{(k)}) = \text{FNN}_p^{(i)}(\xi), \,\xi \sim \mathcal{N}(\mu_v, \Sigma_v), \;  \text{where}\,\mu_v = \text{FNN}_\mu(h_v^{(k)}), \Sigma_v = \text{diag}(\exp(\text{FNN}_\sigma(h_v^{(k)}))).
\end{align*}
The rationale of this setting is due to the universal approximation capability of FNNs to (approximately) reconstruct any distributions in Wasserstein distance~\citep{lu2020universal}, even if the distribution has discrete supports in a continuous space as ours.

A further challenge is that Wasserstein distance between $\mathcal{P}_v^{(i)}$ and $\psi_p^{(i)}(h_v^{(k)})$ does not have a closed form. Therefore, we adopt empirical Wasserstein distance: For every forward pass, the model will get $q$ sampled nodes $\mathcal{N}_v$, denoted by $v_1, v_2,...,v_q$ and thus $\{h_{v_j}^{(i)}|1\leq j\leq q\}$ are $q$ samples from $\mathcal{P}_v^{(i)}$; Next, get $q$ samples from $\mathcal{N}(\mu_v, \Sigma_v)$, denoted by $\xi_1,\xi_2,...,\xi_q$, and thus $\{\hat{h}_{v}^{(i,j)} = \text{FNN}_p^{(i)}(\xi_j)|1\leq j\leq q\}$ are $q$ samples from $\psi_p^{(i)}(h_v^{(k)})$; Adopt the following empirical surrogated loss of $\sum_{i=0}^{k-1}\mathcal{W}_2^2(\mathcal{P}_v^{(i)}, \psi_p^{(i)}(h_v^{(k)}))$ in Eq.\eqref{eq:k-hop-loss},
%$\psi_p^{(i)}(h_v^{(k)})$, denoted by $\hat{h}_{v}^{(i,1)}$, ... , $\hat{h}_{v}^{(i,q)}$, and use the empirical surrogated loss of $\mathcal{W}_2^2(\mathcal{P}_v^{(i)}, \psi_p^{(i)}(h_v^{(k)}))$, \textit{i.e.,}
\begin{align}\label{eq:emp-W-dis}
     \min_{\pi} \sum_{i=0}^{k-1}\sum_{j=1}^q\|h_{v_j}^{(i)}-\hat{h}_{v}^{(i,\pi(j))}\|^2,\;\text{s.t.}\;\pi\;\text{is a bijective mapping:} [q]\rightarrow [q].
\end{align}
Computing the above loss is based on solving a matching problem and needs the Hungarian algorithm with $O(q^3)$ complexity \citep{jonker1987shortest}. More efficient types of surrogate loss may be adopted, such as Chamfer loss based on greedy approximation \citep{fan2017point} or Sinkhorn loss based on continuous relaxation~\citep{cuturi2013sinkhorn}, whose complexities are $O(q^2)$. In our experiments, as $q$ is fixed as a small constant, say $5$, and thus we use Eq.\eqref{eq:emp-W-dis} based on a Hungarian matching that does not introduce much computational overhead. 

Though not directly related, we would like to highlight some recent works that use OT losses as distance between two graphs, where Wasserstein distance between the two sets of node embeddings of these two graphs is adopted~\citep{xu2019gromov,xu2019scalable}. Borrowing such a concept, one can view our OT loss also to measure the distance between the original graph and the decoded graph.   


\subsection{Further Discussion --- Decoders $\psi_s$ and $\psi_d$} \label{sec:further-dis}
The decoder $\psi_s$ to reconstruct the initial features $h_v^{(0)}$ is an FNN. The decoder $\psi_d$ to reconstruct the node degree is an FNN plus exponential neuron to make the value non-negative. 
\begin{align} \label{eq:two-decoder}
    \psi_s(h_v^{(k)}) = \text{FNN}_s(h_v^{(k)}), \quad \psi_d(h_v^{(k)}) = \exp(\text{FNN}_d(h_v^{(k)})).
\end{align}
In practice, the original node features $X$ could be very high-dimensional and reconstructing them directly may introduce a lot of noise into the node representations. Instead, we may first map $X$ into a latent space to initialize $H^{(0)}$. However, if $H^{(0)}$ is used in both representation learning and reconstruction, it has the risk to collapse to trivial points. Hence, we normalize $H^{(0)}=\{h_v^{(0)}|v\in V\}$ properly via pair-norm~\citep{zhao2020pairnorm} to avoid this trap as follows
\begin{align} \label{eq:ini}
   \{h_v^{(0)}|v\in V\} = \text{pair-norm} (\{x_v W|v\in V\}), \; \text{where $W$ is a learnable parameter matrix.}
\end{align}

%Our auto-encoder is generic for any GNN encoders $\phi$ that follow the message passing framework~\citep{gilmer2017neural}. In our experiments, we adopt GCN~\citep{kipf2016semi} and GIN~\citep{xu2018powerful}. 

% to reconstruct the initial features $h_v^{(0)}$ and
% Note that $$



% $\ell_2$-Wasserstein distance for the distribution reconstruction and the squared loss for the node degree reconstruction:



% Based on NID, the neighbor


% %\begin{align}
% \begin{display}
%     \textbf{NID:} \text{Neighborhood information $H^{(0)}_{\mathcal{N}_v}$} is doing $d_v$ times \text{i.i.d.} sampling from $\mathcal{P}_v^{(1)}$,
%     \end{display}
    
%     %\,\text{sampling $d_v$ times,} \stackrel{\text{i.i.d.}}{\sim}
% %\end{align}

% where $\mathcal{P}_v^{(1)}(h):\triangleq \frac{1}{d_v}\sum_{u\in \mathcal{N}_v} \delta(h=h_u^{(0)})  $
% Based on NID, we further write the loss  
% \begin{align} \label{eq:split}
% \mathcal{M}_{n}(H^{(0)}_{\mathcal{N}_v}, \psi(h_v^{(1)})) = 
% \end{align}



%  $\mathcal{P}_v^{(0)}$
% $d_v$

% how to measure the distance to a set     

% and for different nodes, the size of . Here, we decompose the information of  





% %\{h_u^{(0)}|u\in \mathcal{N}_v\}


% % \begin{align*}
% %     \min_{\phi^{(1)},\psi^{(1)}} \sum_{v\in V} \mathcal{M}_s(h_v^{(0)}, \psi^{(1)}(h_v^{(1)}))+ \mathcal{M}_r(\{h_u^{(0)}|u\in \mathcal{N}_v\}, \psi^{(1)}(h_v^{(1)})), \quad \text{s.t. }h_v^{(1)} = \phi^{(1)}((h_v^{(0)}, \{h_u^{(0)}|u\in \mathcal{N}_v\})).
% % \end{align*}



% tuple  $h_v^{(1)} = \phi^{(1)}((h_v^{(0)}, \{h_u^{(0)}|u\in \mathcal{N}_v\}))$


% We consider the following reconstruction loss
% \begin{align*}
%     \min_{\phi^{(1)},\psi^{(1)}} \sum_{v\in V} \mathcal{M}((h_v^{(0)}, \{h_u^{(0)}|u\in \mathcal{N}_v\}), )
% \end{align*}


% Because for every node $v\in V$, $h_v^{(1)} = $


% The architecture of $\psi^{(1)}$ will be introduced in Sec.\ref{sec:decoder}.  Because for every node $v\in V$, $h_v^{(1)} = $

% Consider minimizing the following loss function  


% To simplify the exposition, we fix our discussion to $k$-hop neighborhood reconstruction. Let $G = (V, E, X)$ denote the input graph where $V$ is the node set of size $M$, $E$ is the edge set and $X$ includes the node features $X=\{x_v|v\in V\}$. Given a node $v\in V$, define its $k$-hop neighborhood as $\mathcal{N}_v^{(k)}=\{u\in V| l(u,v)\leq k\}$, where $l(\cdot,\cdot)$ denotes the shortest path distance. Denote the induced $k$-hop subgraph based on $\mathcal{N}_v^{(k)}$ as $G_v^{(k)}$. Note that $G_v^{(k)}$ also contain all the node features in $\mathcal{N}_v^{(k)}$. %Our neighborhood reconstruction principle is defined as 
% Consider a uniform distribution $\mathcal{P}$ over the universe of all possible $k$-hop subgraphes  

% \begin{definition}
% \end{definition}





%  %and later generalize the notion to $k$-hop setting.
% Consider a probability distribution $\mathcal{P}$ defined over a universe $\Omega \triangleq \mathcal{V}\times \mathcal{N}$, where $\mathcal{V}$ is the set of nodes in a graph and $\mathcal{N}$ is the set of posi



% Let $G = (V, E, X)$ denote the input graph where $V$ is the node set of size $N$, $E$ is the edge set and $X\in \mathbb{R}^{N\times F}$ includes the node features. For $v\in V$ $\mathcal{N}_v$



% Suppose we have a set of node features $X = \{x_1, x_2, ..., x_N\}$, where $N$ is the number of nodes in the graphs and each $x_i\in \mathbb{R}^F$.

% Let $G = (V, X, A)$ denote the input graph, where $V$ is the node set of size $N$ and $E$ is the edge set. Let $X\in \mathbb{R}^{N\times F}$ 
% For each node $v\in V$, we define its   

% we are provided with a set
% of node features, X = {~x1, ~x2, . . . , ~xN }, where N is the number of nodes in the graph and ~xi ∈ R
% F
% represents the features of node i. We are also provided with relational information between these
% nodes in the form of an adjacency matrix, A ∈ R
% N×N . While A may consist of arbitrary real
% numbers (or even arbitrary edge features), in all our experiments we will assume the graphs to be
% unweighted, i.e. Aij = 1 if there exists an edge i → j in the graph and Aij = 0 otherwise.
% Our objective is to learn an encoder, E : R
% N×F × R
% N×N → R
% N×F
% 0
% , such that E(X, A) = H =
% {
% ~h1,
% ~h2, . . . ,
% ~hN } represents high-level representations ~hi ∈ R
% F
% 0
% for each node i. These representations may then be retrieved and used for downstream tasks, such as node classification.
% Here we will focus on graph convolutional encoders—a flexible class of node embedding architectures, which generate node representations by repeated aggregation over local node neighborhoods
% (Gilmer et al., 2017). A key consequence is that the produced node embeddings, ~hi
% , summarize a
% patch of the graph centered around node i rather than just the node itself. In what follows, we will
% often refer to ~hi as patch representations to emphasize this point.






% with node feature vector $X(v)$ and neighborhood sets $\mathcal N(v)$ for $v \in V$. We designed a GIN Encoder Network to encode the initial node feature and graph structure information for $G$.

% by investigating the mechanism of GNNs that are to encode the source information  

% much more source information that  

% but simultaneously loses much more information 


% that has been encoded into the latent representations.  


% without exception,

% This may severely affect the quality of the compressed representations.

% To better understand this point, we carefully analyze the source of information encoded in a node    



% almost without exception,

% information reconstruction goal.  


% But this is crucial 


% divergence in opinions appears especially on what information should be reconstructured.  


% Given By minimizing the information loss during the compression, the optimal way for dimension 


% The encoder maps each data point into its latent vector representation embedded in a low dimensional space.



% Following the tradition of dimension reduction, auto-encoders aim to keep the information of the data as much as possible within some latent vector representations that  only a limited budget of dimensions. %Specifically, %an auto-encoder maps each data point into its latent vector representation embedded in a low dimensional space. Au
% To accomplish this task, an auto-encoder consists of two components, an encoder and a decoder. %$\phi$ and a decoder $\psi$. 
% %The encoder maps each data point into a vector in a low dimensional space, termed the latent representation of this data point. 
% The encoder works to compress each data point into a low-dimensional vector, while the decoder works to reconstruct the original information from this vector. Given By minimizing the information loss during the compression, the optimal way for dimension 

% %Typically, they are to solve the problems 
% %\begin{align}
% %    \min_{\phi, \psi} \mathbb{E} d(x - \psi \circ \phi (x) 
% %\end{align}


% that maps a higdata point into a low 
% %which can be viewed as neural-network-based counterparts of principal component analysis (PCA). 

% though auto-encoders have recently been used  
% \subsection{Mingyue-org}

% In this work, we propose an unsupervised structural node representation model that follows a novel design of an jointly encoder-decoder framework. This model leverage the intense proximity preserving power of modern GNNs, and continuously self-refining its structural representations for each node by decoding its neighborhood embedded information. 

% Let $G = (V, E)$ denote an input graph with node feature vector $X(v)$ and neighborhood sets $\mathcal N(v)$ for $v \in V$. We designed a GIN Encoder Network to encode the initial node feature and graph structure information for $G$.

% \subsection{Graph Neural Network Encoder}



% Our Graph Neural Network (GNN) encoder network's goal is to encode the k-hops neighborhood information for each node as an untrained node embedding. For example, the Graph Isomorphism Network (GIN) can be plugged here as a GNN encoder. The GIN encoder iteratively updates node representation by aggregating representations of its neighbors with a multi-layer perceptron (MLP) function. This way, the k-layer encoded node embeddings can capture the structural information within its k-hop network neighborhood. The formal GIN updates node representations can be written as
% \begin{equation}
% h_v^{(k)} = MLP^{(k)} ((1+\epsilon^{k}) \cdot h_v^{(k-1)} + \sum_{u \in \mathcal N(v)} h_u^{k-1} \label{gin-encoder-equation}
% \end{equation}
% In our setting, the $\epsilon$ and MLP parameters are learnable, and the initial (layer 0) node representation $h_v^0 = X(v)$. We take the k layer node embeddings result as an input and other layers embeddings as neighborhood set references for our decoder model. The encoder also can be placed by any types of Graph Convolutional Network (GCN) layer.

% To avoid the encoder be optimized to a trivial solution (all zeros), we add a pair-norm to normalize the outputs of each layer. 
% \begin{equation}
%     h_v^{(k)} = pair-norm(h_v^{(k)})
% \end{equation}
% % \begin{equation}
% % h_v^{(k)} = \sigma(b^(k) + \sum_{j \in \mathcal{N}(i)} \frac{1}{c_{ji}} h_j^kW^k) \label{gcn-encoder-equation}
% % \end{equation}

% % where $\mathcal{N}(i)$ is the neighbors of node i, $c_{ji}$ is the product of the square root of node degrees, and $\sigma$ is an activation function. 
% \begin{figure}
%   \centering
%   \centerline{\includegraphics[width=\columnwidth]{Encoder.png}}  
%   \caption{GNN Encoder Structure, encoding graph into k layers node embeddings}
% \end{figure}

% \subsection{Gaussian Neighborhood Embedding Re-constructor Network}

% \begin{figure}
%   \centering
%   \centerline{\includegraphics[width=\columnwidth]{GNNStructEmbedding.png}}  
%   \caption{Neighborhood Embedding Re-constructor Structure, reconstruct neighborhood embeddings of $v_n$ based on wasserstein distance between the sampled neighborhood embeddings and the ground truth neighborhood embeddings of $v_n$}
% \end{figure}

% The decoder model consists of two parts, 

% 1) \textbf{Node degree decoder}, uses a L layer feed-forward neural network with ReLU activations to predict the degree number $d(v)$ of a given node $h_v^{(k)}$
% \begin{equation}
%     d(v) = W_{l}^T(ReLU(W_{l-1}^T h_v^k + b_{l-1})) + b_l, \quad l \in 1..L \label{degree_decoder}
% \end{equation}
% 2) \textbf{Neighborhood embeddings re-constructor (decoder)}, samples neighborhood embeddings $SN_i(V_n^k)$ for $i \in 1..d(v)$ of a given node $V_n$, then mapping and adjusting the embeddings according to the all previous level reference neighborhood embeddings $h(\mathcal N(v)^{k-1})$

% For the \textbf{Node degree decoder}, let $D(v) = |\mathcal N(v)|$ denotes the ground truth degree of a node v.  The decoder tries to predict the node's degree with a mean squared error loss.
% \begin{equation}
%     L_{nd} = \sum_{v \in V} \frac{(d(v)-D(v))^2}{|V|} \label{degree_loss}
% \end{equation}
% To sample and re-construct the neighborhood embeddings, we introduce our \textbf{neighborhood embeddings re-constructor}, which has a Gaussian distribution sampler with a set matching Hungarian loss-based wasserstein distance. The re-constructor is consist of a Gussian sampler, an non-linear transformation FNN, and a Hungarian matching-based wasserstein distance loss. 
% \begin{equation}
% gd \sim \mathcal N(\mu, \sigma^2), \quad gd \in \mathcal GD \label{normal_distribution}
% \end{equation}
% To construct the neighborhood embeddings of layer $k$ central node $v$, we first sample the neighborhood embedding $ S(h(v)^k)$ by Gussian sampler $ D(v)$ times to generate an approximate neighborhood embeddings matrix $\mathcal SN^k$. Then input the sampled neighborhood embeddings matrix $\mathcal SN^k$ into a non-linear L layer forward-feed network
% \begin{equation}
% \mathcal{LS}N^k = W_{l}^T(ReLU(W_{l-1}^T \mathcal{S}N^k + b_{l-1})) + b_l, \quad l \in 1..L
% \end{equation}
% Where the $W_{l}$ and $b_l$ are learnable parameters, and $LSN^k$ represent the decoded neighborhood embeddings of node $v$. 

% To calculate the distance between decoded neighborhood embeddings $LSN^k$ and reference neighborhood embeddings $h(U)^{k-1}, U \in \mathcal{N}$, we first match every node in $LSN^k$ with nodes in $h(U)^{k-1}$ by Hungarian algorithm and calculate a minimum pair-wise $L_2$ loss to measure the loss of neighborhood re-construction. An example of this matching process can be found at figure. We will prove in Section x that the Hungarian loss here is essentially a wasserstein distance. 

% For Hungarian matching. Both decoded and reference embedding sets have $O(n!)$ permutation probabilities. The matching problem here can be considered as a linear assignment problem, which can be solved by Hungarian Algorithm in $O(n^3)$ times. We use a pairwise Hungarian loss as assignment costs:
% \begin{equation}
% L_{hun}(\mathcal {LS}N^k, h(U)^{k-1}) = min_{\pi \in \Pi} ||\mathcal {LS}N^k_i - h(U)^{k-1}_i||, LSN^k = [LS(h(v)^k)_1...LS(h(v)^k)_{d(v)}]
% \end{equation}
% Where $\Pi$ is the space of permutations, each $\pi$ matches up the element in  $ \mathcal LSN^k$ to the closest element in $ h(U)^{k-1}$.

% The above $L_{hun}$ is for node $v$ in encoder layer $k$, which corresponding to the decoder layer $k-1$. Therefore we need to repeat the whole re-construction $k$ times, the total re-construction loss of node $v$ is 
% \begin{equation}
% L_{recon}(v) = L_{hun}(\mathcal {LS}N^k, h(U)^{k-1}) + L_{hun}(\mathcal {LS}N^{k-1}, h(U)^{k-2}) + \cdots + L_{hun}(\mathcal {LS}N^{1}, h(U)^{0})
% \end{equation}
% The total loss of re-constructing the whole graph $G$ is $L_{recon} = \sum_{v \in V} L_{recon}(v)$. Therefore, the total loss of the decoder network is
% \begin{equation}
%     L_{loss} = \alpha L_{nd} + (1-\alpha) L_{recon}
% \end{equation}
% Where $\alpha$ is a learnable parameter, $L_{nd}$ is the degree loss and $L_{recon}$ is the loss for re-constructing the whole graph $G$. 


% where $(k-1)$ is the number of decoder layer, and $|V|$ is the number of nodes in graph $G$.
% \begin{equation}
%     S(h(v)^k) = \sum_{m=1}^{M} z_m \cdot gd_m \label{sample_func}
% \end{equation}

% For each node v, $z_m$ follows a local multinomial distribution and serves as a categorical variable for multimodal Gaussian distribution combination. We uses a simple L layer FNN + Gumbel softmax network to convert the embedding information to class probabilities then assign the class probabilities $\pi_1 ... \pi_M$ to categorical variables $z_1...z_M$

% \begin{align}
% X = W_{l}^T(ReLU(W_{l-1}^T h_v^k + b_{l-1})) + b_l, \quad l \in 1..L \label{} \\

% \Pi = softmax(X), |\Pi| = M \label{} \\

% z_m = \frac{exp(\frac{log(\pi_i) + g_i}{\tau})}{\sum_{j=1}^M exp(\frac{log(\pi_i) + g_i}{\tau})}, \quad \pi_i, \pi_j \in \Pi, \quad for \quad i = 1..M \label{} \\
% \end{align}

% Where the initial temperature value is 1.0, gradually decreased to 0.3, and $g_1..g_M$ are i.i.d samples drawn from Gumbel(0, 1), which allows us to introduce the randomness to the final categorical variable.

% and there are M independent multivariate Gaussian distributions $gd_m$ which belongs to the same set of distributions $\mathcal GD$

% \begin{equation}
% gd_m \sim \mathcal N(\mu_m, \sigma_m^2), \quad gd_m \in \mathcal GD \label{normal_distribution}
% \end{equation}

% To construct the neighborhood embeddings of layer $k$ central node $v$, we first sample the neighborhood embedding $ S(h(v)^k)$ $ D(v)$ times to generate an approximate neighborhood embeddings matrix $\mathcal SN^k$

% We compare the sampled neighborhood embeddings $\mathcal SN^k$ with the ground truth upper-level node embeddings $h(U)^{k-1}$ , $U=\mathcal N(v)$ . Both embedding sets have $O(n!)$ permutation probabilities. The matching problem here can be considered as a linear assignment problem, which can be solved by Hungarian Algorithm in $O(n^3)$ times. We use a pairwise Hungarian loss as assignment costs:

% $$L_{hun}(\mathcal SN^k, h(U)^{k-1}) = min_{\pi \in \Pi} ||\mathcal SN^k_i - h(U)^{k-1}_i||, \quad  SN^k = [S(h(v)^k)_1...S(h(v)^k)_{d(v)}]$$

% Where $\Pi$ is the space of permutations, each $\pi$ matches up the element in  $ \mathcal SN^k$ to the closest element in $ h(U)^{k-1}$

% Therefore, the total loss of the decoder network is

% $$ L_{loss} = L_{hun}(\mathcal SN^k, h(U)^{k-1}) + L_{nd}$$

% The training process follows a jointly encoder-decoder training manner. All parameters in the encoder network can be learned by minimizing the loss of the whole decoder network. Thus, the optimized encoder network can output adjusted node embeddings that better identify the structure role information after several training batches. 

% \begin{algorithm}[tb]
%   \caption{One forward pass of the GNNStructEmbedding framework within the training loop}
%   \label{alg:example}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} Graph $G=(V, E)$, Node Attributes $X$
%   \STATE $h^1(V)..h^k(V) = GIN^k(G, X)$
%   \FOR{$i=1$ {\bfseries to} $|V|$}
%   \STATE $d_i = DegreeDecoder(h^k(V_i))$
%   \STATE $L_{nd} = MSEloss(d_i, \mathcal N(V_i)) + L_{nd}$
%   \STATE $Z_i = GumbelSoftmax(h^k(V_i))$
%   \STATE $\mathcal{GD}_i \sim Normal(\mu_i, \sigma_i^2)$
%   \FOR{$j=1$ {\bfseries to} $|\mathcal N(V_i)|$}
%   \STATE $\mathcal{SN}_j^k = Z_i \cdot \mathcal{GD}_i$
%   \ENDFOR
%   \STATE $L_{hun} = HungarianLoss(\mathcal{SN}_i^k, h^{k-1}(V_i)) + L_{hun}$
%   \ENDFOR
%   \STATE $\mathcal L_{loss} = L_{nd} + L_{hun}$
% \end{algorithmic}
% \end{algorithm}

%\subsection{Model Optimization}

